Exploring the Open World Using Incremental Extreme Value Machines

Dynamic environments require adaptive applications. One particular machine learning problem in dynamic environments is open world recognition. It characterizes a continuously changing domain where only some classes are seen in one batch of the training data and such batches can only be learned incrementally. Open world recognition is a demanding task that is, to the best of our knowledge, addressed by only a few methods. This work introduces a modification of the widely known Extreme Value Machine (EVM) to enable open world recognition. Our proposed method extends the EVM with a partial model fitting function by neglecting unaffected space during an update. This reduces the training time by a factor of 28. In addition, we provide a modified model reduction using weighted maximum K-set cover to strictly bound the model complexity and reduce the computational effort by a factor of 3.5 from 2.1 s to 0.6 s. In our experiments, we rigorously evaluate openness with two novel evaluation protocols. The proposed method achieves superior accuracy of about 12 % and computational efficiency in the tasks of image classification and face recognition.

==> settings/commands.tex <==
\makeatletter

% requires \usepackage{xspace}
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

% V.C.: I prefer e.\,g., / i.\,e., (the way we were told by US professors ;)
\def\eg{\emph{e.\,g}\onedot} \def\Eg{\emph{E.\,g}\onedot}
\def\ie{\emph{i.\,e}\onedot} \def\Ie{\emph{I.\,e}\onedot}
% V.C.: it is uncommon to write c.f.
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.\,r.\,t\onedot} \def\dof{d.\,o.\,f\onedot}
\def\etal{\emph{et al}\onedot}

% *** NOTATION/SPELLING ***

% Scheirer and others introduced the terms open space, open set, etc. and wrote it like this (without a minus/hyphen)
\def\closedset{closed set\xspace} \def\Closedset{Closed set\xspace}
\def\openset{open set\xspace} \def\Openset{Open set\xspace} \def\OpenSet{Open Set\xspace}
\def\openspace{open space\xspace} \def\Openspace{Open space\xspace}
\def\openworld{open world\xspace} \def\Openworld{Open world\xspace} \def\OpenWorld{Open World\xspace}

\def\fixedsize{fixed-size\xspace} \def\Fixedsize{Fixed-size\xspace}
\def\pseudocode{pseudocode\xspace} \def\Pseudocode{Pseudocode\xspace}
\def\realworld{real-world\xspace} \def\Realworld{Real-world\xspace}
\def\setcover{set cover\xspace} \def\Setcover{Set cover\xspace} \def\SetCover{Set Cover\xspace}
\def\taildistance{tail distance\xspace} \def\Taildistance{Tail distance\xspace}
\def\tailsize{tail size\xspace} \def\Tailsize{Tail size\xspace}
\def\vertexcover{Vertex Cover\xspace}

% *** DATASETS ***
\newcommand{\cifar}[1]{\mbox{CIFAR-\num{#1}}\xspace}
\newcommand{\icdar}{ICDAR\num{17}\xspace}

\newcommand{\protocolA}{Protocol~I\xspace}
\newcommand{\protocolB}{Protocol~II\xspace}

\makeatother

% *** HIGHLIGHT COMMENTS ***
\newcommand{\ch}[1]{\textcolor{violet}{CH: #1}} % Christian
\newcommand{\vc}[1]{\textcolor{cyan}{VC: #1}} % Vincent
\newcommand{\tho}[1]{\textcolor{green}{TH: #1}} % Thomas
\newcommand{\tob}[1]{\textcolor{blue}{TO: #1}} % Tobias

% *** MATH ***
% math simplifications
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\newcommand{\tc}{\text{,}}
\newcommand{\td}{\text{.}}

% vectors/matrices
\newcommand{\BA}{\bm{A}}
\newcommand{\BI}{\bm{I}}
\newcommand{\Bp}{\bm{p}} \newcommand{\BP}{\bm{P}}
\newcommand{\Bx}{\bm{x}} \newcommand{\BX}{\bm{X}}

% Greek vectors/matrices
\newcommand{\Bnu}{\bm{\nu}}

% mathcal/mathbb
\newcommand{\MA}{\mathcal{A}}
\newcommand{\MC}{\mathcal{C}}
\newcommand{\MN}{\mathcal{N}}
\newcommand{\MO}{\mathcal{O}}
\newcommand{\MP}{\mathcal{P}}
\newcommand{\MR}{\mathbb{R}}
\newcommand{\MS}{\mathcal{S}}
\newcommand{\MU}{\mathcal{U}}
\newcommand{\MV}{\mathcal{V}}

% *** OTHER ***
\newcommand{\mytmp}{empty}
\newcommand{\mytmpa}{empty}
\newcommand{\mytmpb}{empty}


\definecolor{my-green}{HTML}{8bda71}
\definecolor{my-yellow}{HTML}{dada71}
\definecolor{my-orange}{HTML}{daa671}
\definecolor{my-red}{HTML}{da7171}

\def\zz#1{%
\ifdim#1pt<25pt\cellcolor{my-green}\else
\ifdim#1pt<50pt\cellcolor{my-yellow}\else
\ifdim#1pt<75pt\cellcolor{my-orange}\else
\cellcolor{my-red}\fi\fi\fi
#1}

